Least Squares Rational Approximation

Rational approximation appears in many contexts throughout science and engineering, playing a central role in linear systems theory, special function approximation, and many others. There are many existing methods for solving the rational approximation problem, from fixed point methods like the Sanathanan-Koerner iteration and Vector Fitting, to partial interpolation methods like Adaptive Anderson Antoulas (AAA). While these methods can often find rational approximations with a small residual norm, they are unable to find optimizers with respect to a weighted l2 norm with a square dense weighting matrix. Here we develop a nonlinear least squares approach constructing rational approximations with respect to this norm. We explore this approach using two parameterizations of rational functions: a ratio of two polynomials and a partial fraction expansion. In both cases, we show how we can use Variable Projection (VARPRO) to reduce the dimension of the optimization problem. As many applications seek a real rational approximation that can be described as a ratio of two real polynomials, we show how this constraint can be enforced in both parameterizations. Although this nonlinear least squares approach often converge to suboptimal local minimizers, we find this can be largely mitigated by initializing the algorithm using the poles of the AAA algorithm applied to the same data. This combination of initialization and nonlinear least squares enables us to construct rational approximants using dense and potentially ill-conditioned weight matrices such as those that appear as a step in new H2 model reduction algorithm recently developed by the authors.

==> alg_grassmann_gn.tex <==
\begin{algorithm}[t]
\begin{minipage}{\linewidth}
\begin{algorithm2e}[H]
\Input{Initial $\ve b_0 \in \C^{n+1}$; backtracking parameter $\gamma \in (0,1)$; \\
	Armijo tolerance $\beta\in (0,1)$}
\Output{Optimized $\ve b \in \C^{n+1}$}
\For{$k=0,1,2,\ldots$}{
	Normalize: $\ve b_k \leftarrow \ve b_k/\| \ve b_k\|_2$\;
	Build residual $\uve r$ and Jacobian $\uve J$ at $\ve b_k$ using \cref{alg:polyJ}\;
	Compute short form SVD: $\uma U\, \uma \Sigma\, \uma V^\trans \leftarrow \uve J$\;
	Compute Gauss-Newton step \cref{eq:poly_gnstep}: 
	$\uve d_k \leftarrow -\sum_{j=1}^{2n} [\uma \Sigma]_{j,j}^{-1} [\uma V]_{\cdot,j} [\uma U^\trans \uve r]_{j}$\;
	\label{alg:grassmann_gn:GNstep}
	Compute slope along Gauss-Newton step: $\alpha \leftarrow \uve d_k^\trans \uve b_k$\;
	\If{$\alpha > 0$}{
		Set step to the negative gradient: $\uve d_k \leftarrow -\uma J^\trans \uve r$\;
		Update slope: $\alpha \leftarrow \uve d_k^\trans \uve b_k$\; 
	}
	Compute norm of step: $\sigma \leftarrow \| \uve d_k\|_2$\; 
	\For{$t = \gamma^0,\gamma^1,\gamma^2,\ldots$}{
		Compute candidate step: $\ve b_+ \leftarrow \ve b_k \cos(\sigma t) + \ve d_k \sin(\sigma t)/\sigma$\;
		Compute candidate residual $\uve r_+$ at $\ve b_+$ using \cref{alg:polyJ}\;
		\lIf{$\|\uve r_+\|_2\le \|\uve r\|_2 + \alpha \beta t$}{{\bf break}}
	}
	Update: $\ve b_{k+1}\leftarrow \ve b_+$\;
}
\end{algorithm2e}
\vspace{-1em}
\end{minipage}
\caption{Grassmann Gauss-Newton for the Polynomial Parameterization}
\label{alg:grassmann_gn}
\end{algorithm}


==> alg_main.tex <==
\begin{algorithm}[t]
\begin{minipage}{\linewidth}
\begin{algorithm2e}[H]
	\Input{Data $\ve z, \ve y$}
	\Output{Local minimizer $\ve\lambda$}
	Form initial estimate via linearization \;
	\For{$k=0,1,2,\ldots$}{
		$\ve r \leftarrow \ve r(\ve \lambda_k; \ve z)$ \;
		$\ma J \leftarrow \ma J(\ve \lambda_k; \ve z)$\;
		$\ve p \leftarrow -\ma J^+\ve r$\;
		$t = 1$\;
		Construct Lagrange polynomial basis $\lbrace \psi_j^{(k)} \rbrace_{j=0}^n$ with nodes at $0$ and $\ve\lambda_k$\;
		\Repeat{until Armjio conditions satisfied}{
			$\ve \lambda_{k+1} \leftarrow \ve\lambda(q(\cdot; t \ma D(\ve e_0)^{-1} \ve p))$\;
			$t \leftarrow t/2$\;
		}
	}
\end{algorithm2e}
\end{minipage}
\caption{Geodesic rational approximation}
\end{algorithm}


==> alg_recursive.tex <==
\begin{algorithm}[t]
\begin{minipage}{\linewidth}
\begin{algorithm2e}[H]
	\Input{Desired degree $(m,n)$, if $r$ should be real}
	\Output{Initial estimate of poles $\ve\lambda$}
	\If{$r$ is real and $n$ is even}{
		$\widehat{n} \leftarrow 2$ \;
		$\widehat{m} \leftarrow$\; 
	}
\end{algorithm2e}
\end{minipage}
\caption{Recursive Initialization}
\end{algorithm}


==> algorithm.tex <==
\section{Algorithm}


\subsection{Proper rational approximation}
We form mismatch this way so that VARPRO reveals a projector.
\begin{equation}
	\minimize_{\ve \lambda, \ve d \in \C^{n} } \| \ve y - \ma C(\ve\lambda) \ve d \|_2^2
\end{equation}

\begin{equation}
	\minimize_{\ve \lambda \in \C^{n} } \| \ma P_{\ma C(\ve\lambda)}^\perp \ve y\|_2^2
\end{equation}

\input{alg_main}

\subsection{Using Demmel to improve accuracy}
$\ma C(\ve\lambda)$ is a Cauchy matrix
and at a critical step, VARPRO requires a projector onto the range of this matrix.
Use~\cite{Dem99} we can compute the SVD of $\ma C(\ve\lambda)$ to high relative accuacy.

\subsection{Extension to improper}
Here we append the matrix $\ma C(\ve\lambda)$
with columns of a Vandermonde matrix to allow $m > n-1$:
\begin{equation}
	\hma C_\ell(\ve\lambda; \ve z) = \begin{bmatrix} \ma C(\ve\lambda; \ve z) & \ma V_{\ell}(\ve z) \end{bmatrix}.
\end{equation}
We loose the ability to apply Demmel, but can now work on a broader class of rational approximation problems. 




==> optimization.tex <==
\section{An Optimization Approach}
Our goal in this section will be to describe how to solve the following 
weighted nonlinear least squares problem:
\begin{equation}
	\minimize_{\ve\theta} \| \ma W[ \ve r(\ve z; \ve\theta) - \ve y] \|_2
\end{equation}
where $\ve r$ is a vector of samples of the rational function $r(z;\ve\theta)$:
\begin{equation}
	\ve r(\ve z; \ve\theta) = \begin{bmatrix} r(z_1;\ve\theta) \\ \vdots \\ r(z_M;\ve\theta)\end{bmatrix}.
\end{equation}

\subsection{Variable Projection}
A key tool we will use in our optimization approach is 
\emph{variable projection} (VARPRO).


\subsection{Choice of Basis}
We have two choices of basis for rational approximation:
pole-residue and polynomial.



\subsubsection{Polynomial Parameterization}



\subsubsection{Pole-Residue Parameterization}
If instead, we use a pole-residue parameterization we are restricted to
rational approximation of degree $(m,n)$ where $m\ge n-1$.


% plot of condition number of basis
%\input{fig_condition}

\subsection{Improper Rational Basis}

\subsection{Nonlinear Trajectory}

%\input{fig_local_minima}

\subsection{Recursive Initialization}
As with any nonconvex optimization algorithm,
a key concern is how to effectively initialize the algorithm.
As illustrated in \cref{fig:local_minima},
the rational fitting problem possesses many local minima
to which the algorithm will converge when initialized randomly.
Here we describe a recursive initialization strategy 
for the rational approximation problem similar to that found in~\cite[Sec.~6.3]{Hok17}.
This approach fits a sequence of lower order rational approximations.


\begin{align}
	\|\ma W[ \diag(\ma \Psi \ve b)^{-1} \ma \Phi\ve a  - \ve h]\|_2 \Longrightarrow
	\| \ma W \ma \Phi \ve a - \ma W \diag(\ma \Psi \ve b) \ve h\|_2 = 
	\left\| \ma W \begin{bmatrix} \ma \Phi & -\diag(\ve h)\ma \Psi \end{bmatrix}
		\begin{bmatrix} \ve a \\ \ve b \end{bmatrix}
	\right\|_2
\end{align}

\input{alg_recursive}



==> param.tex <==
\section{Parameterizations of Rational Functions}
A fundamental choice in rational approximation is the 
parameterization used for the rational approximant.

% Cite DGA10 (p.2739 "Therefore, minimal parameterizations should be avoided and overparameterizations considered.")
% Their basic idea: Jordan form representation is not smooth if converting from A to a Jordan block,
% I want to make the point that although this is true, this is the wrong metric.
% We want to know if parameterization is continuous in the 2-norm on data
% and if the parameterization is dense in the set of rational functions as measured by 2-norm on data.
%
% Strictly speaking, pole residue loses closet-point property in output space


There are two main factors that affect the conditioning of a rational approximation iteration:
the basis for the polynomials and algorithm.
Here we will consider two main parameterizations of the rational approximation $r$:
the \emph{polynomial} parameterization where $p$ and $q$ are written in terms of bases 
$\lbrace \phi_k \rbrace_{k=0}^m$ and $\lbrace \psi_k \rbrace_{k=0}^n$:
\begin{equation}
	r(z; \ve a, \ve b) := \frac{\sum_{k=0}^{m} a_k \phi_k(z)}{\sum_{k=0}^n b_k \psi_k(z)},
\end{equation}
and the \emph{pole-residue} parameterization in terms of poles $\ve\lambda$ and residues $\ve d$
which is restricted to degree $(n-1,n)$ rational approximations:
\begin{equation}
	r(z; \ve \lambda, \ve d) := \sum_{k=1}^n \frac{ d_k }{z - \lambda_k}.
\end{equation}



\subsection{Polynomial}


\subsection{Pole-Residue}




==> polyopt_grassmann.tex <==

leaving an optimization problem over $\ve b$ alone.
However, so doing presents a challenge:
if we scale $\ve b$ the residual remains the same, as $\ve a$ simply gets scaled to compensate.
To correct this we need to introduce a constraint to reduce the degrees of freedom in this problem.
One approach would be to fix a particular value of $\ve b$, e.g., $b_1 = 1$,
or fix the value at a particular point as vector fitting does, setting $q(0) = 1$.
Both approaches could prove problematic if the solution goes to zero there.
Instead, here we will introduce the assumption that $\|\ve b\|_2 = 1$,
which removes that numerical difficulty.
We can interpet this constraint as recasting the optimization problem 
from being over $\ve b\in \C^{n+1}$ to being over a subspace of dimension one in $\C^{n+1}$, 
namely, $\set B \in \set G(\C^{n+1}, 1)$ where $\set G$ denotes the Grassmann manifold. 
Although this requires some modification, 
there is significant structure that can be exploited and that yields a simple optimization problem.




\subsection{Variable Projection}
For the purposes of using variable projection, 
define $\ma \Omega: \C^{n+1} \to \C^{N\times (m+1)}$ 
\begin{equation}
	\ma \Omega(\ve b) := \diag(\ma \Psi \ve b)^{-1} \ma \Phi 
\end{equation}
As before, after applying Variable Projection, 
we reveal an optimization problem over the nonlinear parameters $\ve b$ alone:
\begin{equation}
	\minimize_{\ve b\in \C^{n+1}, \|\ve b\|_2 = 1}
		\| \ma W \ve f - \ma W\ma \Omega(\ve b)[\ma W\ma \Omega(\ve b)]^+[\ma W \ve f]\|_2.
\end{equation}
Then the residual is:
\begin{equation}
	\ve r(\ve b) := \ma P_{\ma W \ma \Lambda(\ve b)}^\perp \ma W \ve f
\end{equation}
and the Jacobian is
\begin{equation}
	[\ma J(\ve b)]_{\cdot,k}
	= - 
		\ma P_{\ma W\ma \Omega(\ve b)}^\perp	
		\frac{\partial \ma W\ma \Omega(\ve  b)}{\partial  b_k}
		[\ma W\ma \Omega(\ve b)]^+\ve f
	-[\ma W\ma \Omega(\ve b)]^{+*}
	\left(\frac{\partial \ma W\ma \Omega(\ve b)}{\partial  b_k}\right)^*
	\ma P_{\ma W\ma \Omega(\ve  b)}^\perp \ve f
\end{equation} 
For this problem, 
\begin{align}
	\frac{\partial \ma \Omega(\ve b) }{\partial b_k} =&
		-\diag(\ma \Psi \ve b)^{-1} \frac{\partial \diag(\ma \Psi \ve b)}{\partial b_k}
		\diag(\ma \Psi \ve b)^{-1} \ma \Phi \\
		=& -\diag(\ma \Psi \ve b)^{-1} \diag(\ma \Psi \ve e_k) \diag(\ma \Psi\ve b)^{-1}\ma \Phi
		= -\diag(\ma \Psi \ve e_k) \diag(\ma \Psi \ve b)^{-2} \ma \Phi.
\end{align}
Unlike with the pole residue parameterization, 
this matrix is dense and so we cannot use the trick used previously to simply the Jacobian construction.
See \cref{alg:polyJ} for instructions on how to construct $\ma J$.

\input{alg_polyJ}

\subsection{Grassmann Optimization}
Optimization on the Grassmann manifold requires several subtile modifications of our algorithms.
First, rather than moving on straight lines as in Euclidean space, 
steps move along geodesics---paths of constant curvature.
In this one dimensional Grassmann manifold case,
if the search direction $\ve d\in \C^{n+1}$ is computed at the current iterate $\ve b_0$ where $\|\ve b_0\|_2 = 1$
and $\ve d^*\ve b_0 = 0$, the next the step is chosen along the trajectory
\begin{equation}
	\ve b(t) = \ve b \cos(\sigma t) + \ve d \sin(\sigma t), \qquad \sigma = \|\ve d\|_2.
\end{equation}
Similarly the formula for the gradient, Jacobian, and Hessian change.
However, this problem shares a similar structure to the ridge approximation problem~\cite{HC18},
namely the Jacobian is in the nullspace of the range of $\ve b$ at the current iterate (see \cref{sec:proof} for a proof).
Hence, invoking the analysis of \cite[sec.~3.2]{HC18}, the Grassmann Gauss-Newton step is:
\begin{equation}\label{eq:poly_gnstep}
	\uve d = -\uma J(\ve b)^+\uve r(\ve b) \qquad \Rank(\uma J) = 2n; 
\end{equation}
namely, since $\uma J(\ve b)$ is structurally has a nullspace of dimension two,
we use the SVD with this rank truncation built in to compute the step $\uve d$.

\input{alg_grassmann_gn}


==> proof.tex <==
\section{Proof of Orthogonality\label{sec:proof}}
\begin{lemma}
	$\uve b^\trans \uma J(\ve b) = \ve 0$
\end{lemma}
\begin{proof}
	Let $\ma K, \ma L\in \C^{N\times (n+1)}$ be defined as in \cref{alg:polyJ}.
	Then, examining the product and absorbing 
	\begin{align}
		\ve b^*\ma K &= \sum_{k=0}^n \conj b_k (\ma I - \ma Q\ma Q^*)\ma W\diag(\ma \Psi \ve e_k)\diag(\ma \Psi \ve b)^{-2} \ma \Phi \ve a \\
			&= (\ma I - \ma Q\ma Q^*)\ma W \diag(\ma \Psi \conj{\ve b} ) \diag(\ma \Psi \ve b)^{-2} \ma \Phi \ve a
	\end{align} 
\end{proof}

